Spectral Analysis for Semantic Segmentation with Applications on Feature Truncation and Weak Annotation

It is well known that semantic segmentation neural networks (SSNNs) produce dense segmentation maps to resolve the objects' boundaries while restrict the prediction on down-sampled grids to alleviate the computational cost. A striking balance between the accuracy and the training cost of the SSNNs such as U-Net exists. We propose a spectral analysis to investigate the correlations among the resolution of the down sampled grid, the loss function and the accuracy of the SSNNs. By analyzing the network back-propagation process in frequency domain, we discover that the traditional loss function, cross-entropy, and the key features of CNN are mainly affected by the low-frequency components of segmentation labels. Our discoveries can be applied to SSNNs in several ways including (i) determining an efficient low resolution grid for resolving the segmentation maps (ii) pruning the networks by truncating the high frequency decoder features for saving computation costs, and (iii) using block-wise weak annotation for saving the labeling time. Experimental results shown in this paper agree with our spectral analysis for the networks such as DeepLab V3+ and Deep Aggregation Net (DAN).

==> figures/acknowledgement.tex <==
\section{Acknowledgement}\label{sec:acknow}
Authors acknowledge the support of the Ministry of Science and Technology of Taiwan (MOST110-2115-M-A49-003-MY2).


==> figures/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
Our proposed spectral analysis for semantic segmentation network correlate CE, IoU score and gradient back-propagation in the spectrum point of view. 
We first explicitly decompose CE and demonstrate the CE is mainly contributed by the low-frequency component of the segmentation maps, which associates with the features in CNNs at the same frequency. Furthermore, we proposed $R(\nu_{max})$ to estimate the sampling efficiency of the low-resolution grid for segmentation maps. 
We test our theory on two applications: feature truncation and block annotation. Our results show that combination of the feature truncation and the network pruning can save computational cost significantly with small accuracy lost. In addition, the block annotation can potentially save more in labeling cost, since the network trained using the block-wise annotation in an efficient low-resolution grid performs close to the original network. The results from our experiments agree with our theoretical predictions based on $R(\nu_{max})$.
Lastly, despite the theoretical analysis and validation in this work, it remains unclear that how to determine the efficient band limit $\nu_{max}$ of the low-resolution grid for various datasets. It would be our future interests to estimate $\nu_{max}$ from the spectrum of groundtruth annotation.

==> figures/exp.tex <==
\section{Validation and Applications}\label{sec:experiments}
This section aims to validate the spectral analysis in section~\ref{sec:method} and further propose the application, including the feature truncation and block-wise annotation. 
In section~\ref{ssec:exp_spec_ce_grad}, we validate the spectral analysis in section~\ref{sec:method}, including the frequency components of CE in Eq.~\ref{Eq:spec_ce_component} and the spectral gradient in Eq.~\ref{Eq:ce_spec_grad}. 
The validation of $\mathcal{L}_{ce}(\nu)$ the frequency components of CE demonstrates that CE is mainly contributed by the low-frequency component while the validation of $\frac{{\partial \mathcal{L}_{ce}(\nu_i)}}{{\partial x(\nu_j)}}$ the spectral gradient shows that it can be well approximated as the delta function as in Eq.~\ref{Eq:ce_spec_grad_ieq0}.
Based on these numeric validations, we identify the efficient low-resolution grids and apply the grids onto the features in CNNs and the groundtruth annotation. This leads us to further propose two applications that down-sample the segmentation maps into low-resolution grids: (1) Feature truncation and (2) Block-wise annotation, which detailed in section~\ref{ssec:exp_feat_trunc} and section~\ref{ssec:exp_blk_annot}, respectively. 

\noindent\textbf{Datasets.}
% \subsubsection{Datasets.}
We examine the experiments upon the following three semantic segmentation datasets: PASCAL semantic segmentation benchmark \cite{everingham2015pascal}, DeepGlobe land-cover classification challenge \cite{demir2018deepglobe} and Cityscapes pixel-level semantic labeling task \cite{cordts2016cityscapes} (denoted as PASCAL, DeepGlobe and Cityscapes respectively). The PASCAL dataset contains 21 categories, 1464 training images, and 1449 validation images; the dataset further augmented by the extra annotations from \cite{BharathICCV2011}. The DeepGlobe dataset contains 7 categories, 803 training images, which are split into 701 and 102 images for training and validation, respectively. The Cityscapes dataset contains 19 categories, 2975 training images, and 500 validation images.

% DeepLab v3+
% \subsubsection{segmentation networks and implementation details.}
\noindent\textbf{segmentation networks and implementation details.} 
In our experiment, we utilize the standard segmentation networks including DeepLab v3+~\cite{chen2018encoder} and Deep Aggregation Net (DAN)~\cite{kuo2018dan}. We adopt the ResNet-101~\cite{he2016deep} pre-trained on ImageNet-1k~\cite{russakovsky2015imagenet} as the backbone of these networks. These networks are trained by the following training policies: For all datasets, the images are randomly cropped to 513$\times$513 pixels and random-flipped in the training stage; the training batch size are 8. For the PASCAL dataset, the network is trained with initial learning rate 0.0007 and 100 epochs; for DeepGlobe dataset, the network is trained with initial learning rate 0.007 and 600 epochs; for Cityscapes dataset, the network is trained with initial learning rate 0.001 and 200 epochs.

\subsection{Validation of Spectral Analysis}\label{ssec:exp_spec_ce_grad}

\subsubsection{Spectral Decomposition of CE.}\label{ssec:exp_spec_ce_grad:ce}
This section aims to demonstrate that CE is mainly contributed by the low-frequency component, as discussed in section~\ref{ssec:method_spectral_ce}, and investigate the efficacy of using the resolution grid for prediction by the modern networks. 
We evaluate $|b(\nu)|$, $|\widehat{y}(\nu)|$, ${\mathcal{L}}_{ce}(\nu)$ and $R({\nu}_{max})$ based on the various segmentation networks (DeepLab v3+ and DAN) and datasets (PASCAL, DeepGlobe and Cityscapes); $|b(\nu)$| and $|\widehat{y}(\nu)|$ are the averaged power spectrum of $b(\nu,c)$ and $\widehat{y}(\nu,c)$ over all semantic classes $c$ respectively. 
The results are shown in Fig.~\ref{Fig:spectral_model_stat}. To monitor the training progress, the evaluation at both the initial and final stages of network training are additionally shown in Fig.~\ref{Fig:spectral_training_stat}. 
Note here the profiles of $|b(\nu)|$ and $|\widehat{y}(\nu)|$ are normalized with respect to their corresponding maximal values for better comparison over datasets.
%
\begin{figure}[h]
    \centering
    % \includegraphics[width=1.0\columnwidth]{figures/model_stat.png} %dc
    \includegraphics[width=0.7\columnwidth]{figures/model_stat.png} %sc
    \caption{The spectral decomposition of CE (${\mathcal{L}}_{ce}(\nu)$), the relative discrepancy of CE ($R({\nu}_{max})$), and the absolute value of spectra ($|b(\nu)|$ and $|\widehat{y}(\nu)|$). The profiles of $|\widehat{y}(\nu)|$, ${\mathcal{L}}_{ce}(\nu)$, and $R({\nu}_{max})$ are evaluated based on DeepLab v3+ and DAN.}
    \label{Fig:spectral_model_stat}
\end{figure}
%
\begin{figure}[h]
    \centering
    % \includegraphics[width=1.\columnwidth]{figures/training_stat.png} % dc
    \includegraphics[width=0.7\columnwidth]{figures/training_stat.png} % sc
    \caption{Spectral Decomposition of CE for DeepLab v3+ and DAN at both initial and final training stages. The notation follows Fig.~\ref{Fig:spectral_model_stat}. The suffix $_{init}$ additionally denotes the profiles of the network at initial stage.}
    \label{Fig:spectral_training_stat}
\end{figure}
The results shown in Fig.~\ref{Fig:spectral_model_stat} indicate that $|\widehat{y}(\nu)|$ is indeed small in the high-frequency region thus leads to small ${\mathcal{L}}_{ce}(\nu)$, as discussed above. These results also support the fact that CE is mainly contributed by the low-frequency components. On the other hands, the results shown in Fig.~\ref{Fig:spectral_training_stat} reveals that the low-frequency components of ${\mathcal{L}}_{ce}(\nu)$ apparently decreases as training progresses, suggesting that the network learns to capture low-resolution-grid more effectively.

\begin{table}[h]
\centering
\caption{Truncated CE and its relative discrepancy with respect to CE under various band limit ${\nu}$, based on the PASCAL, DeepGlobe and Cityscapes datasets.}
\label{table:spectral_stat}
% \resizebox{0.9\columnwidth}{!}{% %dc
\resizebox{0.6\columnwidth}{!}{%sc
\begin{tabular}{clccccc}
\multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{${\nu}_{max}$} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{32} & \multicolumn{1}{c|}{64} & 256 \\ \hline
\multicolumn{7}{c}{DeepLab v3+} \\ \hline
\multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{0.184} & \multicolumn{1}{c|}{0.040} & \multicolumn{1}{c|}{0.017} & \multicolumn{1}{c|}{0.008} & 0 \\
\multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{$R({\nu}_{max})$} & \multicolumn{1}{c|}{0.053} & \multicolumn{1}{c|}{0.017} & \multicolumn{1}{c|}{0.007} & \multicolumn{1}{c|}{0.003} & 0 \\
\multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{1.782} & \multicolumn{1}{c|}{0.517} & \multicolumn{1}{c|}{0.065} & \multicolumn{1}{c|}{0.014} & 0 \\ \hline
\multicolumn{7}{c}{DAN} \\ \hline
\multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{0.197} & \multicolumn{1}{c|}{0.045} & \multicolumn{1}{c|}{0.017} & \multicolumn{1}{c|}{0.008} & 0 \\
\multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{$R({\nu}_{max})$} & \multicolumn{1}{c|}{0.078} & \multicolumn{1}{c|}{0.025} & \multicolumn{1}{c|}{0.009} & \multicolumn{1}{c|}{0.004} & 0 \\
\multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{2.004} & \multicolumn{1}{c|}{0.723} & \multicolumn{1}{c|}{0.153} & \multicolumn{1}{c|}{0.017} & 0
\end{tabular}
% \begin{tabular}{clccccc}
% \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{${\nu}_{max}$} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{32} & \multicolumn{1}{c|}{64} & 256 \\ \hline
% \multicolumn{7}{c}{DeepLab v3+} \\ \hline
% \multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{0.275} & \multicolumn{1}{c|}{0.040} & \multicolumn{1}{c|}{0.018} & \multicolumn{1}{c|}{0.010} & 0 \\
% \multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{$R({\nu}_{max})$} & \multicolumn{1}{c|}{0.102} & \multicolumn{1}{c|}{0.028} & \multicolumn{1}{c|}{0.010} & \multicolumn{1}{c|}{0.005} & 0 \\
% \multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{2.152} & \multicolumn{1}{c|}{0.668} & \multicolumn{1}{c|}{0.146} & \multicolumn{1}{c|}{0.017} & 0 \\ \hline
% \multicolumn{7}{c}{DAN} \\ \hline
% \multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{0.248} & \multicolumn{1}{c|}{0.035} & \multicolumn{1}{c|}{0.019} & \multicolumn{1}{c|}{0.009} & 0 \\
% \multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{$R({\nu}_{max})$} & \multicolumn{1}{c|}{0.081} & \multicolumn{1}{c|}{0.021} & \multicolumn{1}{c|}{0.008} & \multicolumn{1}{c|}{0.004} & 0 \\
% \multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{1.307} & \multicolumn{1}{c|}{0.255} & \multicolumn{1}{c|}{0.029} & \multicolumn{1}{c|}{0.012} & 0
% \end{tabular}
}
\end{table}

Here we further investigate the limitation of the low-resolution grid and the efficient resolution of the features based on $R({\nu}_{max})$ examined in Fig.~\ref{Fig:spectral_model_stat}. For comparison, we examine the numeric value of $R({\nu}_{max})$ in Table~\ref{table:spectral_stat}. Note that ${\mathcal{L}}_{ce}=\widehat{\mathcal{L}}_{ce}(256)$ dues to the image size 513 in our experiments.
Apparently, as the resolution of the grid goes higher, $R({\nu}_{max})$ becomes smaller since more information on high-frequency is captured. More specifically, $R({\nu}_{max})$ dramatically decrease to small values when $\nu > 10$ in all experiments of the trained networks. On the other hand, the segmentation maps predicted by these networks are evaluated on the 129 $\times$ 129 low-resolution grid that corresponds to ${\nu}_{max} = 64$. 
These empirical evidences suggest that the low-resolution grids with $10 < {\nu}_{max} < 64$ could still efficiently sample the segmentation map without significant information loss. These efficient low-resolution grids are further validated on our proposed applications, \ie feature truncation and block-wise annotation, in sections~\ref{ssec:exp_feat_trunc} and section~\ref{ssec:exp_blk_annot}, respectively. 
Besides, it is apparent from Table~\ref{table:spectral_stat} that $R({\nu}_{max})$ on the Cityscapes dataset is significantly larger than that on the PASCAL and DeepGlobe datasets. We shall expect a better efficacy of the feature truncation and the block-wise annotation on the PASCAL and DeepGlobe datasets. 

\subsubsection{Spectral Gradient.}\label{ssec:exp_spec_ce_grad:grad}
We now turn to evaluate the gradient introduced in section~\ref{ssec:method_spec_grad}, including $\frac{\partial y(\nu_i)}{\partial x(\nu_j)}$ in Eq.~\ref{Eq:convlayer_spec_grad} and $\frac{{\partial {\mathcal{L}}_{ce}(\nu_i)}}{{\partial x(\nu_j)}}$ in Eq.~\ref{Eq:ce_spec_grad}. We demonstrate that both $\frac{\partial y(\nu_i)}{\partial x(\nu_j)}$ and $\frac{{\partial {\mathcal{L}}_{ce}(\nu_i)}}{{\partial x(\nu_j)}}$ can be approximated as the delta function.
%
We validate these spectral gradients on the three datasets (PASCAL, DeepGlobe and Cityscapes datasets) and take the spectra of ASPP (atrous spatial pyramid pooling) features in DeepLab v3+ and DAN as our example $x(\nu_j)$. The evaluated $\frac{{\partial {\mathcal{L}}_{ce}(\nu_i)}}{{\partial x(\nu_j)}}$ for DeepLab v3+ and DAN are illustrated in Fig.~\ref{Fig:spec_grad_deeplab} and Fig.~\ref{Fig:spec_grad_dan}, respectively. Besides, we validate $\frac{{\partial y(\nu_i)}}{{\partial x(\nu_j)}}$ for various operations within the decoder module of these networks, including the convolution, ReLU, bilinear up-sampling, where $x(\nu_j)$ and $y(\nu_i)$ denote the input and output spectra for these operations, respectively. These spectral gradients are illustrated in Fig.~\ref{Fig:spec_grad}.
For all the spectral gradients shown in Fig.~\ref{Fig:spec_grad_deeplab}, Fig.~\ref{Fig:spec_grad_dan} and Fig.~\ref{Fig:spec_grad}, the frequency $\nu_i=(0, \frac{M}{4}, \frac{M}{2})$ are evaluated as examples, where $M$ is the size of input features. For each $\nu_i$, we evaluate the spectral gradient for all frequencies $\nu_j$ in region from $0$ to $\frac{M}{2}$. This results in a matrix of spectral gradient for each $\nu_i$, which is shown in each row respectively. In this experiment, we set the size of input feature $M=33$, which actually corresponds to the feature size of the bottleneck of DeepLab v3+ and DAN. 

\begin{figure}[ht]
    \captionsetup[subfigure]{}
    \centering
    % \begin{subfigure}[]{0.9\columnwidth} %dc
    \begin{subfigure}[]{0.45\columnwidth}
        \centering
        % \includegraphics[width=0.6\columnwidth]{figures/spectral_gradient_deeplab.png} %dc
        \includegraphics[width=1.0\columnwidth]{figures/spectral_gradient_deeplab.png} %sc
        \caption{DeepLab v3+}
        \label{Fig:spec_grad_deeplab}
    \end{subfigure}
    % \begin{subfigure}[]{0.9\columnwidth} %dc
    \begin{subfigure}[]{0.45\columnwidth}
        \centering
        % \includegraphics[width=0.6\columnwidth]{figures/spectral_gradient_dan.png} %dc
        \includegraphics[width=1.0\columnwidth]{figures/spectral_gradient_dan.png}
        \caption{DAN}
        \label{Fig:spec_grad_dan}    
    \end{subfigure}
    \caption{The evaluation of spectral gradient ${{\partial {\mathcal{L}}_{ce}(\nu_i)}}/{{\partial x(\nu_j)}}$ for DeepLab v3+ and DAN. The spectral gradient are evaluated based on PASCAL, DeepGlobe and Cityscapes datasets.}
\end{figure}
%
\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.6\columnwidth]{figures/spectral_gradient_unit.png} %dc
    \includegraphics[width=0.45\columnwidth]{figures/spectral_gradient_unit.png}
    \caption{The evaluation of spectral gradient ${{\partial y(\nu_i)}}/{{\partial x(\nu_j)}}$. The spectral gradient for the convolution, ReLU, and bilinear up-sampling operations are denoted as Conv, ReLU, Upsample, respectively.}
    \label{Fig:spec_grad}
\end{figure}

We can see from Fig.~\ref{Fig:spec_grad} that $\frac{{\partial y(\nu_i)}}{{\partial x(\nu_j)}}$ for the convolution, ReLU and bilinear up-sampling are delta function for all $\nu_i$, which is consistent with our discussion for Eq.~\ref{Eq:convlayer_spec_grad}. 
Moreover, clearly from Fig.~\ref{Fig:spec_grad_deeplab} and Fig.~\ref{Fig:spec_grad_dan}, the spectral gradient $\frac{{\partial {\mathcal{L}}_{ce}(\nu_i)}}{{\partial x(\nu_j)}}$ that accumulating all the operations in the decoder module can be well approximated by the delta function. This verifies the approximation of Eq.~\ref{Eq:ce_spec_grad}. 
Also, these results agrees the discussion in section~\ref{ssec:method_spec_grad} that the feature component at frequency $\nu_i$ only affects ${\mathcal{L}}_{ce}(\nu)$ at the frequency near $\nu_i$, which enable us to further consider the removal of redundant high-frequency feature in section~\ref{ssec:exp_feat_trunc}.

\subsection{Application on Feature Truncation}\label{ssec:exp_feat_trunc}
We propose the feature truncation as a model reduction method that reduce the cost of model without degrading the performance. The feature truncation is intuitively performed by removing the high-frequency components of the decoder features $x(\nu)$ acquired from the in the $R(\nu_{max})$ evaluated in section~\ref{ssec:exp_spec_ce_grad:ce}. 
Noting the the segmentation networks typically have huge parameters in encoder while negligible parameters in decoder. However, the computational costs of decoders are often comparable to those of encoders since it up-samples the features for the dense segmentation map and results in large features for computation.
For example, the encoder of DeepLab v3+ has 95.6 billion FLOPs (floating-point operations) and 60.1 million parameters. In contrast, its decoder has 43.4 billion FLOPs while only has 1.3 million parameters. Similarly, the encoder of DAN has 95.6 billion FLOPs with 60.1 million parameters while the decoder has 11.1 billion FLOPs with only 0.4 million parameters.
The truncation of the features in decoder is thus expected to effectively reduce the computational cost. Moreover, one can combine feature truncation with the typical network pruning method to reduce the computation cost in two different aspects, \ie the feature size and the redundant parameters.

We further adopt the Soft Filter Punning (SFP) method~\cite{he2019asymptotic} and combine it with feature truncation as an example. The experiments are done based on the following conditions: For SFP, we use pruning rate [20\%, 40\% and 60\%] for the encoder while use 20\% for the decoder since parameters of the encoder is much larger than that of the decoder and is potentially over-parameterized. 
For the feature truncation applied on the decoder, we down-sample the decoder features from the original size of 129$\times$129 to the efficient low-resolution grids suggested by the analysis in section~\ref{ssec:exp_spec_ce_grad}, \ie the grids with $10 < {\nu}_{max} < 64$. All the down-sampling are done via bilinear interpolation. For simplicity, the experiments mentioned above are only tested on the grid 65$\times$65 and 33$\times$33 that correspond to the band limit ${\nu}_{max}=32$ and ${\nu}_{max}=16$, respectively. The feature size of decoder are [33, 65, 129] in the setup of feature truncation. 
The FLOPs of these experiments are summarized in Table~\ref{table:feat_trunc_flops:flops}, where "Baseline" model denotes the model without SFP. Clearly, the feature truncation effective reduce the FLOPs at various setups of SFP. 
We further evaluate the relative FLOPs-drop, which is the relative deduction rate of FLOPs comparing to that of the model with same SFP setup and the original feature size 129, in Table~\ref{table:feat_trunc_flops:flops_drop}. For example, the relative FLOPs-drop of the setup with "60\% Pruning rate for encoder" and feature size "33" based upon DeepLab v3+ is given as $1-\frac{29}{59}=50.5\%$.
As the feature truncated from 129 to 65, the relative FLOPs-drop are 23.3\% and 7.9\% for the "Baseline" model of DeepLab v3+ and DAN, respectively. As the pruning rate of encoder goes to 60\%, the relative FLOPs-drop even increases to 50.5\% and 24.9\% for the two models, respectively. Recalls that the number parameters of decoder are 1.3 and 0.4 million for the two models. These results actually suggest that the cost reduction rates from feature truncation depend on the number parameters in the decoder. The more parameters in the decoder, the better efficacy of feature truncation is achieved. These results demonstrate an effective cost reduction combining the pruning method (SFP) and feature truncation.
%
\begin{table}[h]
\centering
% \begin{subtable}[]{0.765\linewidth} %dc
\begin{subtable}[]{0.45\linewidth} %sc
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{cccc}
        \hline \multicolumn{4}{c}{DeepLab v3+} \\ \hline
        SFP setups \textbackslash Feature size & 129 & 65 & 33 \\ \hline
        \multicolumn{1}{c|}{Baseline} & 139 & 107 & 98 \\
        \multicolumn{1}{c|}{20\% Pruning rate for encoder} & 100 & 76 & 70 \\
        \multicolumn{1}{c|}{40\% Pruning rate for encoder} & 77 & 53 & 47 \\
        \multicolumn{1}{c|}{60\% Pruning rate for encoder} & 59 & 35 & 29 \\ \hline
        \multicolumn{4}{c}{DAN} \\ \hline
        SFP setups \textbackslash Feature size & 129 & 65 & 33 \\ \hline
        \multicolumn{1}{c|}{Baseline} & 107 & 98 & 96 \\
        \multicolumn{1}{c|}{20\% Pruning rate for encoder} & 78 & 70 & 69 \\
        \multicolumn{1}{c|}{40\% Pruning rate for encoder} & 55 & 47 & 46 \\
        \multicolumn{1}{c|}{60\% Pruning rate for encoder} & 37 & 29 & 28
    \end{tabular}
    }
    \caption{FLOPs for the models with SFP and feature truncation; denoted in unit of $10^9$ FLOPs}
    \label{table:feat_trunc_flops:flops}
\end{subtable}

% \begin{subtable}[]{0.9\linewidth} %dc
\begin{subtable}[]{0.55\linewidth} %sc
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{cccc}
        \hline \multicolumn{4}{c}{DeepLab v3+} \\ \hline
        SFP setups \textbackslash Feature size & 129 & 65 & 33 \\ \hline
        \multicolumn{1}{c|}{Baseline} & 0.0\% & 23.3\% & 29.2\% \\
        \multicolumn{1}{c|}{20\% Pruning rate for encoder} & 0.0\% & 23.7\% & 29.8\% \\
        \multicolumn{1}{c|}{40\% Pruning rate for encoder} & 0.0\% & 30.9\% & 38.7\% \\
        \multicolumn{1}{c|}{60\% Pruning rate for encoder} & 0.0\% & 40.3\% & 50.5\% \\ \hline
        \multicolumn{4}{c}{DAN} \\ \hline
        SFP setups \textbackslash Feature size & 129 & 65 & 33 \\ \hline
        \multicolumn{1}{c|}{Baseline} & 0.0\% & 7.9\% & 9.8\% \\
        \multicolumn{1}{c|}{20\% Pruning rate for encoder} & 0.0\% & 9.4\% & 11.7\% \\
        \multicolumn{1}{c|}{40\% Pruning rate for encoder} & 0.0\% & 13.4\% & 16.7\% \\
        \multicolumn{1}{c|}{60\% Pruning rate for encoder} & 0.0\% & 19.9\% & 24.9\%
    \end{tabular}
    }
    \caption{Relative FLOPs-drop caused by feature truncation.}
    \label{table:feat_trunc_flops:flops_drop}
\end{subtable}
\caption{FLOPs reduction.}
\label{table:feat_trunc_flops}
\end{table}
%
\begin{table*}[h]
\centering
% \begin{subtable}[h]{0.7\textwidth} %dc
\begin{subtable}[h]{0.9\textwidth} %sc
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{ccccccc}
    \hline
    Feature & \multicolumn{2}{c|}{PASCAL} & \multicolumn{2}{c|}{DeepGlobe} & \multicolumn{2}{c}{Cityscapes} \\ \cline{2-7} 
    size & mIoU & \multicolumn{1}{c|}{relative mIoU-drop} & mIoU & \multicolumn{1}{c|}{relative mIoU-drop} & mIoU & relative mIoU-drop \\ \hline
    \multicolumn{7}{c}{Baseline} \\ \hline
    \multicolumn{1}{c|}{129} & 78.6\% & \multicolumn{1}{c|}{0.0\%} & 53.9\% & \multicolumn{1}{c|}{0.0\%} & 67.8\% & 0.0\% \\
    \multicolumn{1}{c|}{65} & 78.1\% & \multicolumn{1}{c|}{0.6\%} & 53.6\% & \multicolumn{1}{c|}{0.6\%} & 62.7\% & 7.4\% \\
    \multicolumn{1}{c|}{33} & 75.6\% & \multicolumn{1}{c|}{3.8\%} & 53.1\% & \multicolumn{1}{c|}{1.5\%} & 53.3\% & 21.3\% \\ \hline
    \multicolumn{7}{c}{20\% Pruning rate for encoder} \\ \hline
    \multicolumn{1}{c|}{129} & 76.6\% & \multicolumn{1}{c|}{0.0\%} & 53.7\% & \multicolumn{1}{c|}{0.0\%} & 67.2\% & 0.0\% \\
    \multicolumn{1}{c|}{65} & 76.0\% & \multicolumn{1}{c|}{0.8\%} & 53.4\% & \multicolumn{1}{c|}{0.7\%} & 62.4\% & 7.1\% \\
    \multicolumn{1}{c|}{33} & 73.2\% & \multicolumn{1}{c|}{4.4\%} & 52.7\% & \multicolumn{1}{c|}{2.0\%} & 53.4\% & 20.5\% \\ \hline
    \multicolumn{7}{c}{40\% Pruning rate for encoder} \\ \hline
    \multicolumn{1}{c|}{129} & 74.4\% & \multicolumn{1}{c|}{0.0\%} & 53.0\% & \multicolumn{1}{c|}{0.0\%} & 66.1\% & 0.0\% \\
    \multicolumn{1}{c|}{65} & 73.9\% & \multicolumn{1}{c|}{0.7\%} & 52.7\% & \multicolumn{1}{c|}{0.6\%} & 61.5\% & 7.0\% \\
    \multicolumn{1}{c|}{33} & 72.1\% & \multicolumn{1}{c|}{3.1\%} & 52.0\% & \multicolumn{1}{c|}{1.9\%} & 52.8\% & 20.1\% \\ \hline
    \multicolumn{7}{c}{60\% Pruning rate for encoder} \\ \hline
    \multicolumn{1}{c|}{129} & 65.1\% & \multicolumn{1}{c|}{0.0\%} & 50.1\% & \multicolumn{1}{c|}{0.0\%} & 58.6\% & 0.0\% \\
    \multicolumn{1}{c|}{65} & 64.7\% & \multicolumn{1}{c|}{0.6\%} & 49.9\% & \multicolumn{1}{c|}{0.4\%} & 54.8\% & 6.5\% \\
    \multicolumn{1}{c|}{33} & 63.3\% & \multicolumn{1}{c|}{2.8\%} & 49.4\% & \multicolumn{1}{c|}{1.4\%} & 47.4\% & 19.2\%
    \end{tabular}
    }
    \caption{DeepLab v3+}
    \label{table:feat_trunc:deeplab}
\end{subtable}

% \begin{subtable}[h]{0.7\textwidth} %dc
\begin{subtable}[h]{0.9\textwidth} %sc
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{ccccccc}
    \hline
    Feature & \multicolumn{2}{c|}{PASCAL} & \multicolumn{2}{c|}{DeepGlobe} & \multicolumn{2}{c}{Cityscapes} \\ \cline{2-7} 
    size & mIoU & \multicolumn{1}{c|}{relative mIoU-drop} & mIoU & \multicolumn{1}{c|}{relative mIoU-drop} & mIoU & relative mIoU-drop \\ \hline
    \multicolumn{7}{c}{Baseline} \\ \hline
    \multicolumn{1}{c|}{129} & 78.7\% & \multicolumn{1}{c|}{0.0\%} & 53.6\% & \multicolumn{1}{c|}{0.0\%} & 66.4\% & 0.0\% \\
    \multicolumn{1}{c|}{65} & 77.9\% & \multicolumn{1}{c|}{1.0\%} & 53.3\% & \multicolumn{1}{c|}{0.5\%} & 61.0\% & 8.1\% \\
    \multicolumn{1}{c|}{33} & 74.5\% & \multicolumn{1}{c|}{5.4\%} & 52.7\% & \multicolumn{1}{c|}{1.7\%} & 50.0\% & 24.8\% \\ \hline
    \multicolumn{7}{c}{20\% Pruning rate for encoder} \\ \hline
    \multicolumn{1}{c|}{129} & 76.8\% & \multicolumn{1}{c|}{0.0\%} & 53.6\% & \multicolumn{1}{c|}{0.0\%} & 65.8\% & 0.0\% \\
    \multicolumn{1}{c|}{65} & 75.9\% & \multicolumn{1}{c|}{1.1\%} & 53.2\% & \multicolumn{1}{c|}{0.8\%} & 60.3\% & 8.3\% \\
    \multicolumn{1}{c|}{33} & 72.8\% & \multicolumn{1}{c|}{5.2\%} & 52.4\% & \multicolumn{1}{c|}{2.2\%} & 49.0\% & 25.5\% \\ \hline
    \multicolumn{7}{c}{40\% Pruning rate for encoder} \\ \hline
    \multicolumn{1}{c|}{129} & 74.6\% & \multicolumn{1}{c|}{0.0\%} & 52.3\% & \multicolumn{1}{c|}{0.0\%} & 65.1\% & 0.0\% \\
    \multicolumn{1}{c|}{65} & 73.8\% & \multicolumn{1}{c|}{1.0\%} & 51.9\% & \multicolumn{1}{c|}{0.8\%} & 59.8\% & 8.1\% \\
    \multicolumn{1}{c|}{33} & 71.3\% & \multicolumn{1}{c|}{4.4\%} & 50.7\% & \multicolumn{1}{c|}{2.9\%} & 48.9\% & 24.9\% \\ \hline
    \multicolumn{7}{c}{60\% Pruning rate for encoder} \\ \hline
    \multicolumn{1}{c|}{129} & 65.6\% & \multicolumn{1}{c|}{0.0\%} & 49.5\% & \multicolumn{1}{c|}{0.0\%} & 57.0\% & 0.0\% \\
    \multicolumn{1}{c|}{65} & 65.1\% & \multicolumn{1}{c|}{0.7\%} & 49.4\% & \multicolumn{1}{c|}{0.3\%} & 52.4\% & 8.1\% \\
    \multicolumn{1}{c|}{33} & 63.0\% & \multicolumn{1}{c|}{3.9\%} & 48.9\% & \multicolumn{1}{c|}{1.4\%} & 42.8\% & 24.9\%
    \end{tabular}
    }
    \caption{DAN}
    \label{table:feat_trunc:dan}
\end{subtable}

\caption{Results for feature truncation and network pruning on DeepLab v3+ and DAN. 
    We summarize the results of using 4 setups of network pruning: "Baseline" denote the experiment without SFP while "X pruning rate for encoder" denotes that with SFP where X = (20\%, 40\%, and 60\%) are the pruning rates. 
    For each setup of network pruning, we further evaluate the results with 3 feature sizes for feature truncation, \ie (129,65,33).}
\label{table:feat_trunc}
\end{table*}
%
\begin{figure}[h]
    \centering
    % \includegraphics[width=1.\columnwidth]{figures/feature_truncation_iou_R.png} %dc
    \includegraphics[width=0.7\columnwidth]{figures/feature_truncation_iou_R.png} %sc
    \caption{The correlation between relative mIoU-drop and the $R(\nu_{max})$ for the feature truncation. The results are evaluated based on PASCAL, DeepGlobe and Cityscapes datasets.}
    \label{Fig:feature_truncation_iou_R}
\end{figure}
%
\begin{figure}[h]
\captionsetup[subfigure]{}
\centering
% \begin{subfigure}[ht]{1.0\columnwidth} %dc
\begin{subfigure}[ht]{0.7\columnwidth}
    \centering
    \includegraphics[width=1.\columnwidth]{figures/feature_truncation_DeepLab.png}  
    \caption{DeepLab v3+}
    \label{Fig:flops_per_iou_deeplab}
\end{subfigure}
% \begin{subfigure}[ht]{1.0\columnwidth} %dc
\begin{subfigure}[ht]{0.7\columnwidth}
    \centering
    \includegraphics[width=1.\columnwidth]{figures/feature_truncation_DAN.png}
    \caption{DAN}
    \label{Fig:flops_per_iou_dan}
\end{subfigure}
\caption{ 
The FPI for DeepLab v3+ and DAN with various prune rates of SFP and feature size (\ie 33, 65, 129) for the feature truncation.}
\label{Fig:flops_per_iou}
\end{figure}

On the other hand, such huge cost reduction indispensably degrade the model performance. Table~\ref{table:feat_trunc:deeplab} and Table~\ref{table:feat_trunc:dan} summarize the performance of DeepLab v3+ and DAN, respectively. These models are evaluated upon the PASCAL, DeepGlobe and Cityscapes datasets. For the experiment upon each dataset, the "mIoU" and "relative mIoU-drop" are evaluated, where "mIoU" is the mean IoU score over all semantic classes; "relative mIoU-drop" is the relative deduction rate of mIoU with respect to that of the model with same SFP setup and feature size 129. 
Apparently from the tables, the mIoU decreases as either the pruning rate increases or as the feature size decreases. Closer inspection of these tables show that the relative mIoU-drop of the experiments on the Cityscapes dataset are significantly larger than that on the PASCAL and DeepGlobe datasets. Taking the "Baseline" model of DeepLab v3+ with feature size 65 as an example, the relative mIoU-drop is 0.6\% for both PASCAL and DeepGlobe datasets, while becomes 7.4\% for the Cityscapes datasets. The same trends holds for the experiments with other SFP setup and feature size based on DeepLab v3+. Also, the similar results are observed in the experiment on DAN as shown in Table~\ref{table:feat_trunc:dan}. 
These significant mIoU-drop on Cityscapes is well explained by the theoretical estimation $R({\nu}_{max})$ in Table~\ref{table:spectral_stat}, where $R({\nu}_{max})$ depict the relative loss of CE evaluated that positively correlates to relative mIoU-drop as discussed in section~\ref{ssec:method_spectral_ioU}. We further illustrate the correlation between the relative mIoU-drop (cf. Table~\ref{table:feat_trunc}) and $R({\nu}_{max})$ (cf. Table~\ref{table:spectral_stat}) in Fig.~\ref{Fig:feature_truncation_iou_R}; where we plot the data with ${\nu}_{max}=[16,32,256]$. The positive correlation in the figure agrees our theoretical statement.
To further estimate the efficiency of these models that simultaneously includes the cost and performance, we define \textbf{FLOPs per IoU score (FPI)} as FLOPs/mIoU. 
The lower the FPI, the better the efficiency of the model that minimizes the performance drop while maximizes the cost reduction of inference.
The FPI of the models in Table~\ref{table:feat_trunc:deeplab} and Table~\ref{table:feat_trunc:dan} are illustrated in Fig.~\ref{Fig:flops_per_iou_deeplab} and Fig.~\ref{Fig:flops_per_iou_dan} for DeepLab v3+ and DAN, respectively.
For the experiments on PASCAL and DeepGlobe datasets, the FPI decreases as feature truncated from 129 to either 65 or 33. In comparison, the decrements of FPI on the Cityscapes dataset is apparently smaller than those on the other datasets. Moreover, the FPI instead increases as feature truncated from 129 to 33 for the experiment of DAN on the Cityscapes dataset. 
These results consist with our analysis on $R({\nu}_{max})$ discussed in section~\ref{ssec:exp_spec_ce_grad}. On the other hand, the results indicates that the feature truncation effectively reduce the computational cost on PASCAL and DeepGlobe datasets with significant reduction of FPI.

% To this end, we demonstrate that the model integrating feature truncation and SFP can effectively reduce the computational cost while keep the performance on some of datasets. The performance drop caused by feature truncation can even correlates to our theoretical analysis.
In summary, we conclude that the integration of feature truncation and SFP can efficiently reduce the computational cost when $R({\nu}_{max})$ is small as demonstrated on the PASCAL and DeepGlobe datasets. On the other hand, it becomes inefficient when $R({\nu}_{max})$ is relatively large as demonstrated on the Cityscapes dataset. 
Our theoretical analysis on $R({\nu}_{max})$ can help to estimate the efficacy of feature truncation for neural networks such as DeepLab v3+ and DAN. To our understanding, this is the first work that provide a theoretical framework to analyze the segmentation performance in the aspect of the frequency domain.
As mentioned in section~\ref{sec:intro}, the existing segmentation networks predict the segmentation maps upon the low-resolution grid to save the computational cost. Our framework serves as a analysis tool to estimate the efficient low-resolution grid size of segmentation maps as well as the effective features in decoders in saving the computational cost. Furthermore, such analysis can be further generalized to arbitrary features in CNNs.

\subsection{Application on Block-wise annotation}\label{ssec:exp_blk_annot}
In section~\ref{ssec:exp_spec_ce_grad}, we determine the efficient low-resolution grid for the segmentation maps via analyzing $R({\nu}_{max})$. In this section, we apply these low-resolution grids to the groundtruth annotations. The resulted block-wise annotation can be considered as a weak annotation. We demonstrate that the performance of the semantic segmentation network trained with these block-wise annotations can also be estimated by $R({\nu}_{max})$.
%
We perform the experiment that trains DeepLab v3+ and DAN with the block-wise annotation at various band limit $\nu_{max}$ (from 8 to 256) and evaluates the $R({\nu}_{max})$ based on the original pixel-wise annotation. Examples of the block-wise annotation and the prediction of the two models upon the PASCAL, DeepGlobe and Cityscapes datasets are illustrated in Fig.~\ref{Fig:block_annotation}. Note that the block-wise annotation at ${\nu}_{max}=256$ is actually equivalent to the original pixel-wise groundtruth. The experimental results are summarized in Table~\ref{table:blk_annot}. For each $\nu_{max}$, we evaluate mIoU score and mIoU drop. Particularly, mIoU-drop is the reduction rate of mIoU with respect to the one band limit ${\nu}_{max}=256$, where this reduction actually corresponds to the decrements of IoU score caused by the low-resolution grid on the annotation.
%
\begin{figure}[h]
    \centering
    % \begin{subfigure}[b]{.9\columnwidth} %dc
    \begin{subfigure}[b]{.6\columnwidth} %sc
        \centering
        \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}[b]{@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}}
            \hline
             $\nu_{max}$ & 256 & 32 & 16 & 8 \\
             \hline
            \multicolumn{5}{c}{PASCAL} \\ \hline  \includegraphics[width=.15\columnwidth]{figures/pascal/voc_image.png} &
            \includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr1_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr8_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr16_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr32_label.png} \\
            \centered{DeepLab v3+} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr1_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr8_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr16_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr32_deeplab.png}} \\
            \centered{DAN} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr1_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr8_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr16_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/pascal/voc_lr32_dan.png}} \\ \hline
            %
            \multicolumn{5}{c}{DeepGlobe} \\ \hline
            \includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_image.png} &
            \includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr1_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr8_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr16_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr32_label.png} \\  
			\centered{DeepLab v3+} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr1_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr8_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr16_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr32_deeplab.png}} \\
			\centered{DAN} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr1_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr8_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr16_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/deepglobe/dg_lr32_dan.png}} \\ \hline
            %
            \multicolumn{5}{c}{Cityscapes} \\ \hline
            \includegraphics[width=.15\columnwidth]{figures/cityscapes/city_image.png} &
            \includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr1_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr8_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr16_label.png} &
            \includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr32_label.png} \\  
			\centered{DeepLab v3+} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr1_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr8_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr16_deeplab.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr32_deeplab.png}} \\
			\centered{DAN} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr1_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr8_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr16_dan.png}} &
            \centered{\includegraphics[width=.15\columnwidth]{figures/cityscapes/city_lr32_dan.png}}
        \end{tabular}
        }
    \end{subfigure}
    \caption{Examples of the block-wise annotation and the prediction of DeepLab v3+ and DAN. For each dataset, the block-wise groundtruth annotations and the predictions of DeepLab v3+ and that of DAN are shown. The corresponding band limits $\nu_{max}$ are denoted at the top of annotation.}
    \label{Fig:block_annotation}
\end{figure}
%
\begin{table}[h]
\centering
% \begin{subtable}[]{0.8\linewidth} %dc
\begin{subtable}[]{0.5\linewidth} %sc
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{ccccc}
    \multicolumn{1}{c|}{${\nu}_{max}$} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{32} & 256 \\ \hline
    \multicolumn{5}{c}{DeepLab v3+} \\ \hline
    \multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{c|}{68.2\%} & \multicolumn{1}{c|}{74.6\%} & \multicolumn{1}{c|}{77.5\%} & 78.6\% \\
    \multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{51.4\%} & \multicolumn{1}{c|}{53.5\%} & \multicolumn{1}{c|}{53.6\%} & 53.9\% \\
    \multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{c|}{38.5\%} & \multicolumn{1}{c|}{50.0\%} & \multicolumn{1}{c|}{59.3\%} & 67.8\% \\ \hline
    \multicolumn{5}{c}{DAN} \\ \hline
    \multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{c|}{68.7\%} & \multicolumn{1}{c|}{74.6\%} & \multicolumn{1}{c|}{77.7\%} & 78.7\% \\
    \multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{50.0\%} & \multicolumn{1}{c|}{52.2\%} & \multicolumn{1}{c|}{53.3\%} & 53.6\% \\
    \multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{c|}{38.4\%} & \multicolumn{1}{c|}{50.1\%} & \multicolumn{1}{c|}{58.5\%} & 66.4\%
    \end{tabular}
    }
    \caption{mIoU score.}
    \label{table:blk_annot:iou}
\end{subtable}

% \begin{subtable}[]{0.8\linewidth} %dc
\begin{subtable}[]{0.5\linewidth} %sc
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{ccccc}
    \multicolumn{1}{c|}{${\nu}_{max}$} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{32} & 256 \\ \hline
    \multicolumn{5}{c}{DeepLab v3+} \\ \hline
    \multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{c|}{13.2\%} & \multicolumn{1}{c|}{5.1\%} & \multicolumn{1}{c|}{1.4\%} & 0.0\% \\
    \multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{4.6\%} & \multicolumn{1}{c|}{0.7\%} & \multicolumn{1}{c|}{0.6\%} & 0.0\% \\
    \multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{c|}{43.2\%} & \multicolumn{1}{c|}{26.3\%} & \multicolumn{1}{c|}{12.5\%} & 0.0\% \\ \hline
    \multicolumn{5}{c}{DAN} \\ \hline
    \multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{c|}{12.7\%} & \multicolumn{1}{c|}{5.2\%} & \multicolumn{1}{c|}{1.3\%} & 0.0\% \\
    \multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{6.7\%} & \multicolumn{1}{c|}{2.6\%} & \multicolumn{1}{c|}{0.7\%} & 0.0\% \\
    \multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{c|}{42.2\%} & \multicolumn{1}{c|}{24.5\%} & \multicolumn{1}{c|}{11.8\%} & 0.0\%
    \end{tabular}
    % \begin{tabular}{ccccc}
    % \multicolumn{1}{c|}{${\nu}_{max}$} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{32} & 256 \\ \hline
    % \multicolumn{5}{c}{DeepLab v3+} \\ \hline
    % \multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{c|}{10.4\%} & \multicolumn{1}{c|}{4.0\%} & \multicolumn{1}{c|}{1.1\%} & 0\% \\
    % \multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{2.5\%} & \multicolumn{1}{c|}{0.4\%} & \multicolumn{1}{c|}{0.3\%} & 0\% \\
    % \multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{c|}{29.3\%} & \multicolumn{1}{c|}{17.8\%} & \multicolumn{1}{c|}{8.5\%} & 0\% \\ \hline
    % \multicolumn{5}{c}{DAN} \\ \hline
    % \multicolumn{1}{c|}{PASCAL} & \multicolumn{1}{c|}{10.0\%} & \multicolumn{1}{c|}{4.1\%} & \multicolumn{1}{c|}{1.0\%} & 0\% \\
    % \multicolumn{1}{c|}{DeepGlobe} & \multicolumn{1}{c|}{3.6\%} & \multicolumn{1}{c|}{1.4\%} & \multicolumn{1}{c|}{0.3\%} & 0\% \\
    % \multicolumn{1}{c|}{Cityscapes} & \multicolumn{1}{c|}{28.0\%} & \multicolumn{1}{c|}{16.3\%} & \multicolumn{1}{c|}{7.9\%} & 0\%
    % \end{tabular}
    }
    \caption{relative mIoU-drop.}
    \label{table:blk_annot:iou_drop}
\end{subtable}
\caption{Experimental results of using our proposed block-wise annotation for learning semantic segmentation based on PASCAL, DeepGlobe and Cityscapes datasets.}
\label{table:blk_annot}
\end{table}
%
As the band limit ${\nu}_{max}$ goes lower, mIoU score goes smaller and a positive mIoU drop is observed. Here we also observe a significant larger amount of mIoU drop on the Cityscapes dataset comparing to those on the PASCAL and DeepGlobe datasets, which is similar to the trend in Flops-drop discussed in previous section. Additionally, such trend consists to the trend of $R(\nu_{max})$ in Table~\ref{table:spectral_stat}, where $R(\nu_{max})$ is significantly larger on the Cityscapes dataset.
% For the experiments on the DeepLab v3+ with $\nu_{max}=32$, the relative mIoU drops are 1.1\%, 0.3\% and 8.5\% on the PASCAL, DeepGlobe and Cityscapes datasets, respectively. Such trend consists to the trend of $R(\nu_{max})$ in Table~\ref{table:spectral_stat}, where 
% $R(32)$ are 0.018, 0.010 and 0.146 for these datasets, respectively. 
% A similar correlation are also observed in the experiments with $\nu_{max}=16$ where the relative mIoU drops are 4.0\%, 0.4\% and 17.8\% and the $R(16)$ are 0.040, 0.028 and 0.668 for these datasets, respectively. 
Fig.~\ref{Fig:block_annotation_iou_R} illustrates the correlation between relative mIoU drops and $R(\nu_{max})$ for all experiments. The positive correlation between mIoU drop and $R(\nu_{max})$ again agrees the correlation between CE and IoU score discussed in section~\ref{ssec:method_spectral_ioU}. Our studies show that the performance of the semantic segmentation network trained with the block-wise annotation strongly correlates to $R(\nu_{max})$. As a result, one can estimate the performance of the semantic segmentation network trained with the block-wise annotation by simply evaluating $R(\nu_{max})$ without thoroughly performing the experiments over all band limits.
%
\begin{figure}[h]
    \centering
    % \includegraphics[width=1.\columnwidth]{figures/block_annotation_iou_R.png} %dc
    \includegraphics[width=0.7\columnwidth]{figures/block_annotation_iou_R.png} %sc
    \caption{The correlation between relative IoU-drop and the $R(\nu_{max})$ for block-wise annotation. The results are evaluated based on PASCAL, DeepGlobe and Cityscapes datasets.}
    \label{Fig:block_annotation_iou_R}
\end{figure}

In summary, the proposed spectral analysis enables the advanced analysis of weak annotation in the frequency domain. Our studies reveal the correlation between the segmentation performance and the low-resolution grid of segmentation maps. Based on our analysis and experiments, the block-wise annotation can be considered as a weak annotation when the block size is chosen according to the size of low-resolution grid in the segmentation maps. Notably, these low-resolution grids actually corresponds to the coarse contour of instances in the segmentation maps, which are greatly utilized in the existing weak annotation. It should be noted that we aim to provide the theoretical justification of the weak annotations by using our spectral analysis. Further research should be undertaken to investigate the spectral analysis upon the existing weak annotations~\cite{papandreou2015weakly,khoreva2017simple} in the future.


==> figures/intro.tex <==
\section{Introduction}\label{sec:intro}
%
Semantic segmentation, which densely assigns semantic labels to each image pixel, is one of the important topics in computer vision. Recently we have witnessed that the CNNs based on the encoder-decoder architecture~\cite{long2015fully,chen2018encoder,badrinarayanan2017segnet, zhao2017psp,chen2014semantic,yang8578486,noh7410535,yu2015multi,PENG2020107498,ZHANG2021107885,ORSIC2021107611,ZHANG2021107940} achieve striking performance on several segmentation benchmarks~\cite{mottaghi2014role,everingham2015pascal,cordts2016cityscapes,zhou2017ade,caesar2018coco}. 
Generally, an encoder-decoder architecture consists of an encoder module that gradually reduces the spatial resolution of features for extracting  context information and a decoder module that aggregates the information from the encoder and gradually recovers the spatial resolution of the dense segmentation map. 
The existing works, \eg Fully Convolutional Neural Network (FCN)~\cite{long2015fully}, U-Net \cite{ronneberger2015u}, and DeepLab models~ \cite{chen2014semantic,chen2017rethinking,chen2018encoder}, utilize encoder-decoder architecture to resolve the dense map. Usually, 
extra modules such as dense conditional random field (dense CRF)~\cite{chen2014semantic,krahenbuhl2011efficient} and PointRend~\cite{kirillov2019pointrend} can be applied to boost the edge-response near object boundaries. On the other hand, most of the above mentioned methods predict the dense segmentation map on a \textbf{low-resolution grid (LRG)}, \eg $\frac{1}{4}$ and $\frac{1}{8}$ of the original image resolution, which is then up-sampled to the original image resolution, to save the computational cost~\cite{chen2018encoder,long2015fully}. \\
%Improving the edge-response at the object boundaries remains a challenge of the existing segmentation networks.}
% Among these works, Long \etal first propose Fully Convolutional Neural Network (FCN)~\cite{long2015fully} that predicts the dense segmentation map by utilizing the skip-architecture, where the features of different granularities in the encoder are up-sampled and integrated in the decoder. The similar idea can also be observed in the U-Net \cite{ronneberger2015u}, which further adds dense skip-connections between the corresponding down-sampling and up-sampling modules of the same feature dimensions.
% Based on such a skip-architecture, Chen \etal propose the DeepLab models~ \cite{chen2014semantic,chen2017rethinking,chen2018encoder} that integrate the atrous spatial pyramid pooling module (ASPP) and the dense conditional random field (dense CRF)~\cite{krahenbuhl2011efficient}, where the former utilizes the dilated convolutional layer composed of the filters at multiple sampling rates while the later one serve as an extra module to boost the edge-response at object boundaries. 
% Similarly, Kirillov \etal~\cite{kirillov2019pointrend} propose the PointRend module as an extra module that adaptively refines the segmentation map by extra point-wise predictions upon the object boundaries. Improving the edge-response at the object boundaries remains a challenge of the existing segmentation networks. 

Besides the LRG for prediction, some of networks can learn sufficient semantic contents from the weak annotations including the pixel level annotation with the coarse contours of objects~\cite{papandreou2015weakly,dai2015boxsup,khoreva2017simple,GUO2021108063,LU2021107924} or those derived from the image level annotation~\cite{ahn2018learning,jing2019coarse,zhou2019wails,shimoda2019self,sun2019fully,nivaggioli2019weakly}. These works demonstrate that networks can still achieve comparable accuracy with those networks that learn from the pixel-wise groundtruth annotation. 
These results indicate that 
\begin{enumerate}
    \item The major semantic contents in segmentation maps can be learned by the existing segmentation networks using the low-resolution annotation in training. % low-freq is important
    \item Despite the inaccurate object boundaries of the weak annotations in the training data set, the  networks are able to predict most of the major components of the objects. % high-freq is not important
\end{enumerate}
In other word, by using proper LRG and weak annotation (WA), one can save costs in labeling and training process without losing too much on the prediction accuracy. To further reduce the cost of inference, network pruning (NP)~\cite{liu2018rethinking,he2019asymptotic,Molchanov_2019_CVPR,blalock2020state,zhao2019variational,luo2017thinet,karnin1990simple} is usually considered where the redundant network parameters are removed if either its contribution to output~\cite{Molchanov_2019_CVPR,luo2017thinet,zhao2019variational} or its norm~\cite{he2019asymptotic} is negligible. 
Despite the success on using LRG, WA and NP for cost saving, it yet remains unclear how these approaches affect the accuracy of the trained networks in theory. In this work, we present a theoretical analysis on the influence of the LRG to the network prediction and identify important features through our theoretical results. We aim to determine an efficient LRG that minimize the performance drop while maximize the cost reduction of training and annotation. 
%
Here note that the LRG is not necessary limited to the network prediction but can be extended to the features in networks or annotation. Our analysis provides an general discussion of the LRG for network prediction, network features (\ie CNN features) and annotation. Besides, we demonstrate that a more effective cost reduction can be made by combing existing pruning methods and features truncation for network inference based on the chosen efficient LRG. Furthermore, we investigate various block-wise annotations that is associated with the chosen LRG in order to alleviate the heavy cost of pixel level annotation. \\

Recently, the spectral analysis on neural networks for fitting uniformly distributed one dimensional signal have demonstrated that the network tends to learn the low-frequency component of target signal in the regression of the uniformly distributed data with various frequencies~\cite{rahaman2018spectral,ronen2019convergence,luo2019theory,yang2019fine}. Such tendency is also known as spectral bias~\cite{rahaman2018spectral}. 
The spectral bias is also observed when we train the segmentation networks, where the semantic contents is mainly learned through coarse contour in WA on the LRG. Hence, we suspect that the WA and LRG actually associates with the low-frequency component of segmentation maps. On the other hand, the noise near object boundary might associates with the high-frequency component of segmentation maps. To verify our speculation on the spectral bias of segmentation networks, we would like to perform a spectral analysis on a semantic segmentation network in section~\ref{sec:method}.
The correlations among the frequency distributions of ground truth annotation and network output segmentation, the objective function (\eg cross-entropy (CE)), the evaluation metric (intersection-over-union (IoU) score), and the resolution of CNN features shall be evaluated in the frequency domain. This further allow us to estimate the \textbf{sampling efficiency} of CNN features, \ie the variation of network performance with respect to the band limit of LRG, and determine the best size of the low resolution grid.
%
In summary, our analysis demonstrates the following key observations:
\begin{itemize}
\item The cross-entropy (CE) can be explicitly decomposed into the summation of frequency components. We find that CE is mainly contributed by the low-frequency component of the ground truth annotation and segmentation maps.
\item Frequency analysis of the IoU score reveals its close relation to the CE. This justifies the CE objective for training the segmentation networks. 
\item The correlation between the segmentation logits and the features within CNNs, in the frequency domain, shows that the segmentation logits of a specific frequency are mainly affected by the features within the same frequency.
\item Based on the findings above, the high frequency components of smooth features are found to be less important. Truncating these high frequency components does not interfere the performance of semantic segmentation networks.
\end{itemize}
\noindent Our findings above contribute to the semantic segmentation networks in the following two objectives:
\begin{enumerate}
    \item \textbf{Feature truncation for segmentation networks.} The features in the decoder can be truncated since they are generally assumed to be smooth comparing to the ones in the encoder. This truncation method can be easily integrated with the commonly-used pruning approaches~\cite{liu2018rethinking,he2019asymptotic} for further cost reduction. Moreover, one can determine the efficient size of LRG by validating the sampling efficiency of CNN feature in spectral analysis.
    \item \textbf{Block-wise annotation.} For semantic segmentation, it is easier to collect a weak annotation that keeps the low-resolution information of the full pixel-wise ground truth annotation. The block-wise annotation can be directly associated with the low frequency spectral information. We propose a block-wise annotation that emulating the existing weak annotations, where only the coarse contours of the instances in the segmentation map~\cite{papandreou2015weakly,khoreva2017simple} are used, and show that the segmentation networks trained via these block-wise annotations are still efficient and accurate. 
\end{enumerate}
Applications related to the above objectives will be shown and discussed in section~\ref{sec:experiments}. The experimental results are expected in our analysis.



==> figures/method.tex <==
\section{Proposed Spectral Analysis}\label{sec:method}
%
As motivated above, we aim to conduct the spectral analysis on segmentation networks and investigate the sampling efficiency of the networks.
To clearly depict the sampling efficiency of the networks, we analyze the formalism of cross-entropy (CE) objective function and the intersection-over-union (IoU) evaluation metric in frequency domain. We demonstrate the analysis of CE in section \ref{ssec:method_spectral_ce} while relegate the analysis of IoU in section~\ref{ssec:method_spectral_ioU} of appendix.
Our results show the positive correlation between IoU score and CE, that justify the usage of CE as objective function and IoU as evaluation metric in the network training framework. Moreover, as CE is decomposed into the components of frequencies, we investigate the learning mechanism for various frequency component. We deduce the gradient propagation for convolutional layers in frequency domain and demonstrate the correlation between the segmentation output and the features in CNNs in section \ref{ssec:method_spec_grad}.  
Our results suggest that the high-frequency components of the features and annotations have less influence on the performance of the segmentation networks due to the band limit introduced by the LRG. Finally, we conclude the spectral analysis upon segmentation networks in section~\ref{ssec:method_discussion}.\\
\\
% \subsubsection{Notation}
\noindent\textbf{Notation}. 
The notations in this section are defined as follows. In general, the upper case letter, \eg $X, Y, Z, B$, denote the functional in the spatial domain $t$ while the lower case letter \eg $x, y, z, b$, denote the corresponding spectrum in the frequency domain $\nu$. For example, the spectrum $y(\nu)=\mathcal{F}(Y(t))$ where  $\mathcal{F}$ is the Fourier transform operator. The rest of notations will be defined whenever they appear.

\subsection{Spectral Decomposition of Cross-Entropy}\label{ssec:method_spectral_ce}
Let $Y(t,c)$ denote the segmentation logits produced by a semantic segmentation network and $B(t,c)$ denote the groundtruth annotation, in which $c$ and $t$ are indexes for the object class and image pixel respectively. The commonly-used objective function for learning semantic segmentation, cross-entropy (CE), can be written as
\begin{equation}
    \begin{aligned}
         \mathcal{L}_{CE} & = -  { \sum _{c}} {\int} B(t,c) {log} (   { \frac {e^{Y(t,c)}}{{ \sum _{c}} e^{Y(t,c)}}}) dt 
        %  \\ & =  -   { \sum _{c}} {\int} B(t,c)(Y(t,c) - {log}({\sum _{c}} e^{Y(t,c)}))dt  
        \\ & = - { \sum _{c}} {\int} B(t,c)(Y(t,c) - {Y_{p}}(t))dt,
    \end{aligned}
    \label{Eq:ce}
\end{equation}
where ${Y_{p}}(t)={log}({ \sum _{c}} e^{Y(t,c)})$. Transforming this integral into frequency domain $\nu$ give theorem~\ref{theorem:ce}.
%
\begin{restatable}[Spectral decomposition of Cross-Entropy]{theorem}{ce}
\label{theorem:ce}
% \begin{theorem}\label{theorem:ce}
Given $Y$ the segmentation logits and $B$ the groundtruth annotation, the cross-entropy $\mathcal{L}_{CE}$ can be decomposed as $\mathcal{L}_{CE} = {\sum _{\nu}} \mathcal{L}_{ce}(\nu)$, where $\mathcal{L}_{ce}(\nu)$ is the \textbf{frequency components of CE} and can be computed as following,
\begin{equation}
    \begin{aligned}
        \mathcal{L}_{ce}(\nu) = { \sum_{c} }{b}(-\nu, c)({y_{p}}(\nu) - y(\nu, c))
    \end{aligned}
    \label{Eq:spec_ce_component}
\end{equation}
here, $b, y,$ and $y_{p}$ are the spectra of $B, Y,$ and $Y_{p}$, respectively. 
% \end{theorem}
\end{restatable}

\begin{proof}
Given $Y$ and $B$, $\mathcal{L}_{CE}$ the cross-entropy is
\begin{equation}
    \begin{aligned}
         \mathcal{L}_{CE} & = -  { \sum _{c}} {\int} B(t,c) {log} (   { \frac {e^{Y(t,c)}}{{ \sum _{c}} e^{Y(t,c)}}}) dt 
        %  \\ & =  -   { \sum _{c}} {\int} B(t,c)(Y(t,c) - {log}({\sum _{c}} e^{Y(t,c)}))dt  
        \\ & = - { \sum _{c}} {\int} B(t,c)(Y(t,c) - {Y_{p}}(t))dt,
    \end{aligned}
    % \label{Eq:ce}
\end{equation}
where ${Y_{p}}(t)={log}({ \sum _{c}} e^{Y(t,c)})$. 
For all $Y(t)\in  Y(t,c)$ and ${B}(t)\in B(t,c)$, the integral ${\int} Y(t){B}(t)dt$ can be transformed to the frequency domain $\nu$ as follows. (See lemma~\ref{lemma:ft_prod} of appendix)
\begin{equation}
    \begin{aligned}
        {\int} Y(t){B}(t)\,dt = {\int} y(z)\,{b}( - z)\,dz
    \end{aligned}
\end{equation}
where $y(\nu)$ and $b(\nu)$ are the spectrum of the segmentation logits and that of the groundtruth annotations, respectively. The $\mathcal{L}_{CE}$ in Eq.~\ref{Eq:ce} is hence given by
\begin{equation}
    \begin{aligned}
         \mathcal{L}_{CE} & = - { \sum _{c}} {\int} B(t,c)(Y(t,c) - {Y_{p}}(t))dt
              \\ & = { \sum _{c}} {\int} {b}(-\nu, c)({y_{p}}(\nu) - y(\nu, c))d\nu.
    \end{aligned}
    \label{Eq:spectral_ce_final}
\end{equation}
The discrete integral of  Eq.~\ref{Eq:spectral_ce_final} gives us the  decomposition of the $\mathcal{L}_{CE}$  over frequency domain $\nu$ as following
\begin{equation}
    \begin{aligned}
        \mathcal{L}_{CE} & = { \sum _{\nu}} { \sum_{c} }{b}(-\nu, c)({y_{p}}(\nu) - y(\nu, c))
          \\ & = { \sum _{\nu}} \mathcal{L}_{ce}(\nu),
    \end{aligned}
    \label{Eq:spec_ce_final_discrete}
\end{equation}
where 
\begin{equation}
    \begin{aligned}
        \mathcal{L}_{ce}(\nu) = { \sum_{c} }{b}(-\nu, c)({y_{p}}(\nu) - y(\nu, c)).
    \end{aligned}
    % \label{Eq:spec_ce_component}
\end{equation}
\end{proof}
%
The contribution from each frequency components to CE can thus be evaluated. In addition, it follows immediately that $\mathcal{L}_{ce}(\nu)$ is small when either ${y_{p}}(\nu) - y(\nu, c)$ or $b(\nu,c)$ is small. For simplicity, let $\widehat{y}(\nu,c) = {y_{p}}(\nu) - y(\nu, c)$. Recalls that, as mentioned in section~\ref{sec:intro}, $Y(t,c)$ is generally predicted upon the low-resolution grid. Hence, $\widehat{y}(\nu_i,c)$, as well as $\mathcal{L}_{ce}(\nu_i)$, should be small at high-frequency $\nu_i$. 
Besides, the magnitude of high frequency components of the ground truth annotation is generally small dues to the intrinsic smoothness of segmentation map~\footnote{Segmentation map usually consists of several segment for each class. All the internal region of segment is flat while only the regions near the  segmentation boundaries contain high-frequency components.}
One can therefore conclude that $\mathcal{L}_{CE}$ is the mainly contributed by the low-frequency components. This conclusion will be validated later in section~\ref{ssec:exp_spec_ce_grad} and lead us to the first key observation.
Furthermore, it follows from this observation that the significance of high-frequency component of pixel-wise groundtruth to $\mathcal{L}_{CE}$ is negligible. This also explain why weak annotation, which drop the high-frequency component of segmentation map, can be an effective approach to pixel-wise groundtruth annotation. Most of researches in studying weak annotations~\cite{papandreou2015weakly,dai2015boxsup,khoreva2017simple,GUO2021108063,LU2021107924,ahn2018learning,jing2019coarse,zhou2019wails,shimoda2019self,sun2019fully,nivaggioli2019weakly} demonstrate efficacy of WA solely by experiments on benchmark datasets. Here, our spectral analysis further provide a theoretical foundation to the WA.

Besides the analysis of CE, we further perform the analysis of IoU score and correlate it to the analysis of  CE in section~\ref{ssec:method_spectral_ioU}. The analysis reveals how the minimization of CE correlates to the maximization of IoU score. This observation justifies the rationality of the common learning procedure for semantic segmentation networks: the networks are trained by the CE objective function while being validated by the IoU scores.
This corresponds to the second key observation. Therefore, later in our experiments and analysis, we adopt the decomposition of CE to study the frequency response and take IoU as a reasonable metric for evaluation.

\subsection{Spectral Gradient of Convolutional Layers}\label{ssec:method_spec_grad}
In section~\ref{ssec:method_spectral_ce}, we have demonstrated that the CE can be decomposed into the summation of frequency components $\mathcal{L}_{ce}(\nu)$. Here we further deduce the gradient propagation of $\mathcal{L}_{ce}(\nu)$ within CNNs in order to reveal how $\mathcal{L}_{ce}(\nu)$ updates the network, especially for the gradient in low-frequency regime. 
% Recalls that the low-frequency component of segmentation map are generally utilized such as the down-sampled grid of the network prediction and the weak annotation. \textcolor{red}{We'd therefore focus how the low-frequency components of segmentation map are affected by the features in CNNs as  frequency region varies during the back-propagation.}
We hereafter refer the gradient propagation with respect to input feature $X$ in frequency domain as the \textbf{spectral gradient}. With this, we can analyze how the low-frequency of input feature affect the network performance. For simplicity, we deduce the spectral gradient for a convolutional layer, including a convolution and an activation function
\begin{equation}
    \begin{aligned}
        Z(t) & = K(t) \otimes X(t)
        \\ Y(t) & =\sigma(Z(t)),
    \end{aligned}
    \label{Eq:conv_layer}
\end{equation} 
where $K$ is the kernel, $\sigma$ is the activation function, $X$ is input feature, and $Y$ is the output of convolutional layer. We consider the soft-plus activation $\sigma(Z(t)) = \log ( {1 + {e^{Z(t)}}}) $ since its everywhere differentiable thus make it easier for analysis. 
The spectral gradient for a convolutional layer is given as below.
\begin{restatable}[The spectral gradient for a convolutional layer]{theorem}{ce_grad}
\label{theorem:ce_grad}
Given $B$ the groundtruth annotation, $X$, $K$ and $Y$ as in Eq.~\ref{Eq:conv_layer}, the spectral gradient of $\mathcal{L}_{ce}(\nu)$ the frequency components of CE is 
\begin{equation}
    \begin{aligned}
        \frac{{\partial \mathcal{L}_{ce}(\nu_i)}}{{\partial x(\nu_j)}} 
         \simeq & \sum _c \frac{1}{2}k(\nu_j,c)[D_{0}(\nu_i) s(-\nu_j, c) - \delta_{\nu_j}(\nu_i)b(-\nu_i,c)],
    \end{aligned}
\label{Eq:ce_spec_grad}
\end{equation}
and the spectral gradient of $y$ the output is
\begin{equation}
    \begin{aligned}
         \frac{\partial y(\nu_i)}{\partial x(\nu_j)} \simeq \frac{1}{2}k( \nu_j){{\delta}_{\nu_j}(\nu_i)},
    \end{aligned}
\label{Eq:convlayer_spec_grad}
\end{equation}
% \end{theorem}
assuming the $K(t)$ is small and $|X(t)| < 1$;\footnote{These assumptions rely on the fact that the numeric scale of feature and kernel are usually limited to a small range of value for the numeric stability of networks.} where $y(\nu) = {\cal F}(Y(t))$, $b(\nu) = {\cal F}(B(t))$, $k(\nu) = {\cal F}(K(t))$, $x(\nu) = {\cal F}(X(t))$, and $s(\nu) = {\cal F}(S(t))$ the spectrum of segmentation output. ${\delta}_{\nu_j}(\nu_i)$ is the Kronecker delta function, which is here after abbreviated as the delta function, and $D_{0}(\nu_i)$ is the Dirac delta function. 
\end{restatable}
We relegate the proof of Eq.~\ref{Eq:convlayer_spec_grad} in lemma~\ref{lemma:conv_grad} of appendix and that of Eq.~\ref{Eq:ce_spec_grad} in lemma~\ref{lemma:ce_grad} of appendix.
%
% We then derive the spectral gradient for Eq.~\ref{Eq:conv_layer}. That is, the gradient of $y(\nu) = {\cal F}(Y(t))$ with respect to $x(\nu) = {\cal F}(X(t))$, \ie $\frac{\partial y(\nu)}{\partial x(\nu)}$. 
% Assuming the $K(t)$ is small and $|X(t)| < 1$, the gradient of $y$ under frequency $\nu_i$ with respect to the $x$ under frequency $\nu_j$ is written as follows (see lemma~\ref{lemma:conv_grad} of appendix).
% \begin{equation}
%     \begin{aligned}
%          \frac{\partial y(\nu_i)}{\partial x(\nu_j)} \simeq \frac{1}{2}k( \nu_j){{\delta}_{\nu_j}(\nu_i)},
%     \end{aligned}
% \label{Eq:convlayer_spec_grad}
% \end{equation}
Clearly from the theory, the spectral gradient in Eq.~\ref{Eq:convlayer_spec_grad} can be approximated as the delta function, indicating $y(\nu_i)$ is affected only by $x(\nu_i)$ with the same frequency. This corresponds to the third key observation.
% Following the spectral gradient in Eq.~\ref{Eq:convlayer_spec_grad}, we now derive the spectral gradient of $\mathcal{L}_{ce}(\nu)$ with respect to the features in a convolutional layer. 
% For each semantic class $c$ in segmentation maps, let $k(\nu, c)$ and $y(\nu,c)$ denote the spectrum of kernel and that of the segmentation output for a convolutional layer, respectively. 
% By Eq.~\ref{Eq:spec_ce_component} and Eq.~\ref{Eq:convlayer_spec_grad}, the spectral gradient of $\mathcal{L}_{ce}(\nu)$ can be written as follows. (see lemma~\ref{lemma:ce_grad} of appendix)
% \begin{equation}
%     \begin{aligned}
%         \frac{{\partial \mathcal{L}_{ce}(\nu_i)}}{{\partial x(\nu_j)}} 
%          \simeq & \sum _c \frac{1}{2}k(\nu_j,c)[D_{0}(\nu_i) s(-\nu_j, c) - \delta_{\nu_j}(\nu_i)b(-\nu_i,c)],
%     \end{aligned}
% \label{Eq:ce_spec_grad}
% \end{equation}
% where $D_{0}(\nu_i)$ is the Dirac delta function. 
Now, let us further analyze how the variation of feature $ x(\nu_j)$ affect $\mathcal{L}_{ce}(\nu_i)$ based on Eq.~\ref{Eq:ce_spec_grad}. For simplicity, we consider the case $\nu_i \neq 0$ and $\nu_i = 0$ separately. This reveals the contribution of the feature to network performance and provides a guideline for removing the redundant feature. 
For $\nu_i \neq 0$, the gradient becomes 
\begin{equation}
    \begin{aligned}
        \frac{{\partial \mathcal{L}_{ce}(\nu_i)}}{{\partial x(\nu_j)}} 
         \simeq & -\sum _c \frac{1}{2}k(\nu_j,c) \delta_{\nu_j}(\nu_i)b(-\nu_i,c), \text{if~} \nu_j \neq 0,
    \end{aligned}
\label{Eq:ce_spec_grad_ineq0}
\end{equation}
which indicates that the CNN feature $x(\nu_j)$ is affected only by $\mathcal{L}_{ce}(\nu_i)$ with same frequency. 
For $\nu_i = 0$, the gradient consists of additional term $\sum _c \frac{1}{2}k(\nu_j,c)D_{0}(\nu_i) s(-\nu_j, c)$. 
Here recalls that the segmentation map $s(\nu, c)$ is usually predicted upon the low-resolution grid of the original image as mentioned in section \ref{sec:intro}. $s(\nu, c)$ should therefore be smooth so that $s(-\nu_j, c)$ is small when $\nu_j$ is large. 
Hence,
\begin{equation}
    \begin{aligned}
        \frac{{\partial \mathcal{L}_{ce}(\nu_i)}}{{\partial x(\nu_j)}} 
         \ll 1, \text{if~} \nu_j \text{~is large} \text{~and~} \nu_j \neq \nu_i = 0. 
    \end{aligned}
\label{Eq:ce_spec_grad_ieq0}
\end{equation}
It follows from Eq.~\ref{Eq:ce_spec_grad_ineq0} and Eq.~\ref{Eq:ce_spec_grad_ieq0} that the CNN feature $x(\nu_j)$ is affected only by $\mathcal{L}_{ce}(\nu_i)$ with near frequency. 
Thus, removing the features $x(\nu_j)$ at high-frequency $\nu_j$ does not effect $\mathcal{L}_{ce}(\nu_i)$ at low-frequency $\nu_i$. This give us the forth key observation. With this observation, it becomes possible to reduce the feature size of CNN, as well as its high-frequency components, while keep the performance. We further provide the numerical validation of this observation in section~\ref{ssec:exp_spec_ce_grad}.


\subsection{Discussion for Spectral Analysis}\label{ssec:method_discussion}
In this section, we summarize the discussion for the spectral analysis based on the theoretical analysis in the above sections. Recalls in section~\ref{sec:intro}, the segmentation map is usually predicted upon the low-resolution grid of the original image. We here aims to determine the efficient grid size that maximizing the cost reduction while minimizing the accuracy lost.
% It is yet unclear whether this grid is sufficient to capture the most of the information of CE, especially for the object boundary. 
Following the decomposition of CE in Eq.~\ref{Eq:spec_ce_final_discrete}, we define the truncated CE as the frequency components of CE filtered by a low-pass filter, \ie low-resolution grid, with the band limit ${\nu}_{max}$ as follows, 
% \textcolor{red}{(how do we find $\nu_{max}$ in practice?)}
\begin{equation}
    \begin{aligned}
        \widehat{\mathcal{L}}_{CE}({\nu}_{max}) = { \sum _{\nu}^{{\nu}_{max}}} \mathcal{L}_{ce}(\nu),
    \end{aligned}
    \label{Eq:spectral_ce_bandlimit}
\end{equation}
Further, we define 
\begin{equation}
    R({\nu}_{max}) = |1 - \frac{\widehat{\mathcal{L}}_{CE}(\nu_{max})}{\mathcal{L}_{CE}}|
    \label{Eq:r_max}
\end{equation}
as the losses of $\mathcal{L}_{CE}$ due to the truncation at band limit $\nu_{max}$. Hence, an efficient grid can be defined when $R({\nu}_{max})$ is negligible. These derived efficient grids can be applied to either segmentation outputs or groundtruth annotation with the same $R({\nu}_{max})$ by Eq.~\ref{Eq:spec_ce_component}. In addition, these grids can further be applied to the features in CNNs to save computational cost follows from the forth key observation discussed in section~\ref{ssec:method_spec_grad}. 
In the following section, we apply the efficient grids on the features and the groundtruth annotation and validate the positive correlation between the the loss of CE and the loss of IoU score caused by the efficient grids. 
